Exponentially Faster Shortest Paths in the Congested Clique

We present improved deterministic algorithms for approximating shortest paths in the Congested Clique model of distributed computing. We obtain $poly(\log\log n)$-round algorithms for the following problems in unweighted undirected $n$-vertex graphs: -- $(1+\epsilon)$-approximation of multi-source shortest paths (MSSP) from $O(\sqrt{n})$ sources. -- $(2+\epsilon)$-approximation of all pairs shortest paths (APSP). -- $(1+\epsilon,\beta)$-approximation of APSP where $\beta=O(\frac{\log\log n}{\epsilon})^{\log\log n}$. These bounds improve exponentially over the state-of-the-art poly-logarithmic bounds due to [Censor-Hillel et al., PODC19]. It also provides the first nearly-additive bounds for the APSP problem in sub-polynomial time. Our approach is based on distinguishing between short and long distances based on some distance threshold $t = O(\frac{\beta}{\epsilon})$ where $\beta=O(\frac{\log\log n}{\epsilon})^{\log\log n}$. Handling the long distances is done by devising a new algorithm for computing sparse $(1+\epsilon,\beta)$ emulator with $O(n\log\log n)$ edges. For the short distances, we provide distance-sensitive variants for the distance tool-kit of [Censor-Hillel et al., PODC19]. By exploiting the fact that this tool-kit should be applied only on local balls of radius $t$, their round complexities get improved from $poly(\log n)$ to $poly(\log t)$. Finally, our deterministic solutions for these problems are based on a derandomization scheme of a novel variant of the hitting set problem, which might be of independent interest.

==> det-algorithms-old.tex <==
\section{Deterministic Algorithms}
We begin by setting up some notation.
For a set $S$ we denote by $x \sim S$ a uniform sampling from $S$. For a function $\PRG$ and an index $i$, let $\PRG(s)_i$ 
the $\ith{i}$ bit of $\PRG(s)$. 

\begin{definition}[Pseudorandom Generators]
A generator $\PRG \colon \BB^r \to \BB^n$ is an $\epsilon$-pseudorandom
generator (PRG) for a class $\cC$ of Boolean functions if for every $f \in 
\cC$:
$$
|\Exp{x \sim \BB^n}{f(x)} - \Exp{s \sim \BB^r}{f(\PRG(s))}| \le 
\epsilon.
$$
We refer to $r$ as the seed-length of the generator and say $\PRG$ is explicit 
if there is an efficient algorithm to compute $\PRG$ that runs in time 
$poly(n, 1/\epsilon)$.
%We say $\PRG$ $\epsilon$-fools $\cC$ and refer to $\epsilon$ as the error.
\end{definition}

As in \cite{ParterY18}, we use the following from \cite{gopalan2012better} which gives a PRG for the 
family of DNFs with short seed.

\begin{theorem}\label{thm:prg}
For every $\epsilon=\epsilon(n) > 0$, there exists an explicit pseudoranom 
generator, $\PRG 
\colon 	\BB^r \to \BB^n$ that fools all read-once DNFs on $n$-variables with 
error at most $\epsilon$ and seed-length $r = O((\log(n/\epsilon)) \cdot (\log 
\log(n/\epsilon))^3)$.
\end{theorem}
For a given two subsets of vertices $V_1,V_2$, define the \emph{soft-hitting set} function $SH(V_1,V_2)$ by 
$$
SH(V_1,V_2)=
\begin{cases}
0, \text{~~if~~} V_1 \cap V_2 \neq \emptyset\\
|V_1|, \text{~~otherwise.}\\
\end{cases}
$$
\begin{definition}[Soft Hitting Set]
Let $V' \subseteq V$ be a subset of vertices, where each $u \in V'$ has a set $S_u$ with at least $\Delta$ vertices. 
A set of vertices $R$ is \emph{soft hitting set} for $V'$ if:
(i) $|R|=O(n/\Delta)$ and 
(ii) $\sum_{u \in V'} SH(S_u, R)=O(|V'|\cdot \Delta)$. 
\end{definition}
In this section we show:
\begin{lemma}[Det. Construction of Soft Hitting Sets]
Let $V' \subseteq V$ be a subset of vertices where each vertex $u$ knows a set $S_u$ of at least $\Delta$ vertices. There exists an 
$O((\log\log n)^3)$-round deterministic algorithm that computes a soft-hitting subset $Z \subseteq V$ for $V'$. 
\end{lemma}

We first show that a soft hitting set can be obtained using a small random seed, and later explain how to compute it in the \clique model. 
\begin{lemma}\label{lem:hittingrandloglog}[Soft Hitting Set with Small Seed]
Let $S$ be a subset of $[n]$ where $|S|\ge 
\Delta$ for some parameter $\Delta \le n$ and let $c$ be any constant. 
Then, there exists a family of hash functions $\cH= \{h \colon [n] \to \BB \}$ such 
that choosing a random function from $\cH$ takes $r=O(\log n \cdot (\log\log n)^3)$ 
random bits and for $Z_h = \{u \in [n] : h(u)=1 \}$ it holds that:
(i) $\prob{h}{ |Z_h| =O(n/\Delta)} \ge 2/3$, and
(ii) $\Exp{h}{ SH(S,Z_h) }=O(\Delta)$.
\end{lemma}
\begin{proof}
We first describe the construction of $\cH$. Let $p=c'/\Delta$ for some large constant $c'$ (will be set later), and let $\ell=\lfloor \log 1/p \rfloor$. Let 
$\PRG \colon \BB^r \to \BB^{n\ell}$ be the PRG constructed in 
\Cref{thm:prg} for $r=O(\log n\ell \cdot (\log\log n\ell)^3)=O(\log n \cdot 
(\log\log n)^3)$ and for $\epsilon = 1/n^{10c}$. For a string $s$ of length $r$ 
we define 
the hash function $h_s(i)$ as follows. First, it computes $y=\PRG(s)$. 
Then, it interprets $y$ as $n$ blocks where each block 
is of length $\ell$ bits, and outputs 1 if 
and only if all the bits of the $\ith{i}$ block are 1. 
Formally, we define
$
h_s(i) = \bigwedge_{j=(i-1)\ell+1}^{i\ell}\PRG(s)_{j}.
$
We show that properties (i) and (ii) hold for the set $Z_{h_s}$ where $h_s \in 
\cH$. 
We begin with property (i). For $i \in [n]$ let $X_i=h_s(i)$ be a random 
variable where $s \sim \BB^r$. Moreover, let $X=\sum_{i=1}^{n}X_i$. Using this 
notation we have that $|Z_{h_s}|=X$.
Thus, to show property (i), we need to show that
$
\Pr_{s \sim \BB^r}[X = O(n/\Delta)] \ge 2/3.
$
Let $f_i \colon \BB^{n\ell} \to \BB$ be a function that outputs 1 if the 
$\ith{i}$ 
block is all 1's. That is,
$
f_i(y)=\bigwedge_{j=(i-1)\ell+1}^{i\ell}y_{j}.
$
Since $f_i$ 
is a read-once DNF formula we have that
$$
\left |\Exp{y \sim \BB^{n\ell}}{f_i(y)} - \Exp{s \sim \BB^{r}}{f_i(\PRG(s))} 
\right| 
\le \epsilon.
$$
Therefore, it follows that
$$
\E{X} = \sum_{i=1}^{n}\E{X_i} = \sum_{i=1}^{n}\Exp{s \sim 
\BB^{r}}{f_i(\PRG(s))} \le \sum_{i=1}^{n}(\Exp{y \sim \BB^{n\ell}}{f_i(y)} + 
\epsilon) = n(2^{-\ell} + \epsilon) \leq 2c' n/\Delta.$$
Then, by Markov's inequality we get that $\Pr_{s \sim \BB^r}[X > 3\E{X}] 
\le 1/3$ and thus
$$
\prob{s \sim \BB^r}{X \le 6c'\cdot n/\Delta} \ge
1-\prob{s \sim \BB^r}{X > 3\E{X}} \ge 2/3.
$$

We turn to show property (ii). Let $S$ be any set of size at least $\Delta$ and 
let $g \colon \BB^{n\ell} \to 
\BB$ be an indicator function for the event that the set $S$ is covered. That 
is,
$$
g(y) = \bigvee_{i \in S}\bigwedge_{j=(i-1)\ell+1}^{i\ell}y_j.
$$
Since $g$ is a read-once DNF formula, we have that 
\begin{equation}\label{eq:hit}
\left | \prob{y \sim \BB^{n\ell}}{g(y)=0} - \prob{s \sim \BB^{r}}{g(\PRG(s))=0} 
\right| \le \epsilon~.
\end{equation}

Let $q \colon \BB^{n\ell} \to \{0,|S|\}$ be defined as follows: 
$$
q(y)=
\begin{cases}
0, \text{~~if~~} g(y)=0,\\
|S|, \text{~~otherwise.}\\
\end{cases}
$$
Note that $\Exp{y \sim \BB^{n\ell}}{q(y)}=|S|\cdot \prob{y \sim \BB^{n\ell}}{g(y)=0}$ and $\Exp{s \sim \BB^{r}}{q(\PRG(s))}=|S|\cdot \prob{s \sim \BB^{r}}{g(\PRG(s))=0}$. Combining this with Eq. (\ref{eq:hit}) yields that:
\begin{eqnarray}\label{eq:hit-better}
\left | \Exp{y \sim \BB^{n\ell}}{q(y)} - \Exp{s \sim \BB^{r}}{q(\PRG(s))}
\right| &=& |S|\left | \prob{y \sim \BB^{n\ell}}{g(y)=0}-\prob{s \sim \BB^{r}}{g(\PRG(s))=0} \right|
\\&\le& |S|\cdot \epsilon \leq 1/n^{c-1}~.\nonumber
\end{eqnarray}
Therefore to bound $\Exp{s \sim \BB^{r}}{q(\PRG(s))}$ it is sufficient to bound $\Exp{y \sim \BB^{n\ell}}{q(y)}$.
%The probability that $S$ is not hit by a random bit string $y \sim \BB^{n\ell}$ is $(1-p)^|S|$. 
Since all the bits in $y$ are completely independent we have that
\begin{eqnarray*}
\Exp{y \sim \BB^{n\ell}}{q(y)}&=&\prod_i(1-\prob{y \sim \BB^{n\ell}}{f_i(y)})\cdot |S|
\\&= & (1-p)^{|S|}\cdot |S|\leq e^{|S|/\Delta}\cdot |S|= O(\Delta)~.
\end{eqnarray*}
Property (2) follows by combining with Eq. (\ref{eq:hit-better}).
%
%
%
%
%Let $Y_i= \bigwedge_{j=(i-1)\ell+1}^{i\ell}y_j$, and let $Y=\sum_{i \in S}Y_i$. 
%Then 
%$
%\E{Y} = \sum_{i \in S}\E{Y_i} \ge |S| 2^{-\ell} \ge c'|S|/\Delta.
%$
%
%For $y \in \BB^{n\ell}$, let $R(y)=\{ i ~\mid ~ h_s(i)=1\}$ be the set of elected nodes based on $y$.
%Let $q \colon \BB^{n\ell} \to [0, |S|]$ be a function that outputs 0 if $S \cap R(y)\neq \emptyset$ and $|S|$ otherwise. 
%$$
%\left |\Exp{y \sim \BB^{n\ell}}{f_i(y)} - \Exp{s \sim \BB^{r}}{f_i(\PRG(s))} 
%\right| 
%\le \epsilon.
%$$
%
%
%
%Thus, by a Chernoff bound we have that $\Pr[Y = 0 ] \le \Pr[\E{Y} - Y \ge c'\log n ]  \le 1/n^{2c}$, for a large enough constant $c'$ (that depends on $c$). Together, we get that \\
%$
%\Pr_s[ S \cap Z_{h_s} \ne \emptyset ] = \Exp{s \sim \BB^{r}}{g(\PRG(s))} 
%\ge  \Exp{y \sim \BB^{n\ell}}{g(y)} - \epsilon 
%= \prob{y \sim \BB^{n\ell}}{Y \ge 1} - \epsilon 
%%& \ge 1-1/n^{2c}-\epsilon 
%\ge 1-1/n^{c}.
%$
\end{proof}

We next present a deterministic construction of the \emph{soft} hitting set by means of derandomization. The round complexity of the algorithm depends on the number of random bits used by the randomized algorithms.
\begin{theorem}\label{thm:generalderand}
Let $G=(V,E)$ be an $n$-vertex graph, let $V' \subset V$, let $\mathcal{S}=\{S_u \subset V : u \in V'\}$ be a set of subsets such that each vertex $u \in V'$ knows the set $S_u$ and $|S_u| \ge \Delta$, and let $c$ be a constant.
Let $\cH = \{h \colon [n] \to \BB \}$ be a family of hash functions such 
that choosing a random function $h$ from $\cH$ takes $g(n,\Delta)$ 
random bits and for $Z_h = \{u \in [n] : h(u)=0 \}$ it holds that: 
(1) $\pr{ |Z_h|=O(n/\Delta)} \ge 2/3$ and
(2) $\sum_{u \in V'}\left(\pr{Z_h\cap S_u=\emptyset}\cdot |S_u|\right)=O(\Delta \cdot n)$. \\
Then, there exists a deterministic algorithm $\cA_{det}$ that constructs a soft hitting set in $O(g(n,\Delta)/\log n)$ rounds. 
\end{theorem}
\begin{proof}
Our goal is to completely derandomize the process of finding $Z_h$ by using the 
method of conditional expectations. We follow the scheme of 
\cite{Censor-HillelPS16} to achieve this, and define a unified cost function that depends on the two properties of the soft hitting set. %bad events that can occur when using a random seed of size $g=g(n,\Delta)$.  
Let $X=|Z_h|$ and let $Y=\sum_{u \in V'}SH(S_u,Z_h)/\Delta^2$.  Our goal is to find a seed of $g$ bits that minimizes $X+Y$.
Based on Lemma \ref{lem:hittingrandloglog}, $\Exp{h \in \cH}{X+Y}=O(n/\Delta)$. 
Note that the set $Z_h$ that minimizes the above expectation is a soft-hitting set. 


We will then use the method of conditional expectations in order to get an assignment to our $g$ random coins that minimizes $X+Y$. In each step of the method, we run a distributed protocol to compute the conditional expectation. 
Fix a random seed $y$ of length $g$, and a function $h$ chosen from $\cH$ using $y$. 
For every vertex $u$, let $x_u=1$ if $u$ is in $Z_{h}$, and let $y_u=|S_u|/\Delta^2$ if $S_u \cap Z_h=\emptyset$ and $y_0=0$ otherwise. We then have that $\sum x_u+y_u= X+Y$.
 
%We denote by $X_v$ the indicator variable for the event that vertex $v$ adds too many edges.
%Letting $X_u$ be indicator random variable for the event that $S_u$ is not hit 
%by $Z_h$,
%we can write our expectation as follows:
%$
%\E{A}+\E{X_B} = \pr{X_A=1} + SH() = \pr{X_A=1} + \pr{\vee_{u} X_u=1}~$
%Suppose we have a partial assignment to the seed, denoted by $Y$. Our goal is to compute the conditional expectation $\E{X~|~Y}$, which translates to computing $\pr{X_A=1|Y}$ and $\pr{\vee_{u} X_u=1|Y}$. Notice that computing $\pr{X_A=1~|~Y}$ is simple since it depends only on $Y$ (and not on the graph or the subsets $\mathcal{S}$). The difficult part is computing $\pr{\vee_{u} X_u=1|Y}$. 
%
%Instead, we use a pessimistic estimator of $\E{X}$ which avoids this difficult computation. Specifically, we define the estimator:
%$\Psi = X_A + \sum_{u \in V'} X_u.$
%Recall that for any $u \in V'$ for a random $g$-bit length seed, it holds that $\pr{X_u=1}\leq 1/n^c$ and thus by applying a union bound over all $n$ sets, it also holds that
%$\E{\Psi} = \pr{X_A=1} + \sum_u \pr{X_u=1} < 1$.
%
%
%We describe how to compute the desired seed using the method of conditional expectation. We will reveal the assignment of the seed in chunks of $\ell=\lfloor \log n \rfloor$ bits. In particular, we show how to compute the assignment of $\ell$ bits in the seed in $O(1)$ rounds. Since the seed has $g$ many bits, this will yield an $O(g/\log n)$ round algorithm. 

Suppose that we are given a partial assignment to the first $k$ bits in the seed, and let $Q$ be a random variable that denotes the seed conditioned on this prefix. Any vertex can easily compute the conditional
expectation of $\Exp{}{x_u+y_u ~\mid~ Q}$. The reason is that the expectation depends on the probability that $u$ or one of the vertices in $S_u$ joins the soft hitting set. Since $u$ knows all the vertices in $S_u$ it can compute this value. 

Consider the $\ith{i}$ chunk of the seed $Q_i=(q_1,\ldots, q_\ell)$ for $\ell =\lfloor \log n \rfloor$, and assume that the assignment for the first $i-1$ chunks $Q_1\ldots,Q_{i-1}$ have been computed. For each of the $n$ possible assignments to $Q_i$, we assign a vertex $v$ that receives the conditional expectation values $\Exp{}{x_u+y_u~|~Q_1,\ldots,Q_{i}}$ from all vertices $u \in V'$. 
The vertex $v$ then sums up all these values and sends them to a global leader $w$. The leader $w$, using the values it received from all the vertices, can compute $\Exp{}{X+Y~|~Q_1,\ldots, Q_i}$ for each of the possible $n$ assignments to $Q_i$. Finally, $w$ selects the assignment $(q^*_1,\ldots,q^*_\ell)$ that minimizes the expectation, and broadcasts it to all vertices in the graph. After $O(g/\log n)$ rounds $Q$ has been completely fixed such that the cost value of the chosen set $Z$ is at most $O(n/\Delta)$.
\end{proof}
